Integrating LEO Satellites and Multi-UAV Reinforcement Learning for Hybrid FSO/RF Non-Terrestrial Networks

A mega-constellation of low-altitude earth orbit (LEO) satellites (SATs) and burgeoning unmanned aerial vehicles (UAVs) are promising enablers for high-speed and long-distance communications in beyond fifth-generation (5G) systems. Integrating SATs and UAVs within a non-terrestrial network (NTN), in this article we investigate the problem of forwarding packets between two faraway ground terminals through SAT and UAV relays using either millimeter-wave (mmWave) radio-frequency (RF) or free-space optical (FSO) link. Towards maximizing the communication efficiency, the real-time associations with orbiting SATs and the moving trajectories of UAVs should be optimized with suitable FSO/RF links, which is challenging due to the time-varying network topology and a huge number of possible control actions. To overcome the difficulty, we lift this problem to multi-agent deep reinforcement learning (MARL) with a novel action dimensionality reduction technique. Simulation results corroborate that our proposed SAT-UAV integrated scheme achieves 1.99x higher end-to-end sum throughput compared to a benchmark scheme with fixed ground relays. While improving the throughput, our proposed scheme also aims to reduce the UAV control energy, yielding 2.25x higher energy efficiency than a baseline method only maximizing the throughput. Lastly, thanks to utilizing hybrid FSO/RF links, the proposed scheme achieves up to 62.56x higher peak throughput and 21.09x higher worst-case throughput than the cases utilizing either RF or FSO links, highlighting the importance of co-designing SAT-UAV associations, UAV trajectories, and hybrid FSO/RF links in beyond-5G NTNs.

==> Table/Table2.tex <==
\newcolumntype{R}{>{\raggedleft\arraybackslash}X}
\begin{tabularx}{1\linewidth}{l c r}
    \toprule[1pt]
    Types of Decision for Association  & Spectral Efficiency \\
    (Two SATs + Ground Relays) & [bps/Hz] \\     
    \cmidrule(lr){1-1} \cmidrule(lr){2-3}
    % Naive & $1.9721 \times 10^{-3}$ & {\color{gray}($1 \times$)} \\
    Fixed Ground, Competitive & $17.9519 \times 10^{-3}$ & {\color{gray}($9.1 \times$)} \\
    \textbf{Fixed Ground, Cooperative} & $29.3159 \times 10^{-3}$ & {\color{gray}($14.9 \times$)} \\
    \bottomrule[1pt]
\end{tabularx}

==> Table/Table3.tex <==
\newcolumntype{R}{>{\raggedleft\arraybackslash}X}
\begin{tabularx}{1\linewidth}{l c r}
    \toprule[1pt]
    \multirow{2}{*}{Types of Relaying} & Spectral Efficiency \\
     & [bps/Hz] \\     
    \cmidrule(lr){1-1} \cmidrule(lr){2-3}
    Fixed Ground Relay & $29.316 \times 10^{-3}$ & {\color{gray}($1 \times$)} \\
    \textbf{Mobile UAV, Cooperative} & $58.292 \times 10^{-3}$ & {\color{gray}($2.0 \times$)} \\
    \bottomrule[1pt]
\end{tabularx}

==> Table/Table_Association_Trajectory <==
% Generated with rank_based_methods.py
\newcolumntype{R}{>{\raggedleft\arraybackslash}X}
% \newcolumntype{C}{ >{\centering\arraybackslash} m{4cm} }
% \newcolumntype{D}{ >{\centering\arraybackslash} m{1cm} }

% \tablefontsize
\begin{tabularx}{1\linewidth}{Xcccc}
    \toprule[1pt] 
    & $n=200$ ($t = 2000$ [sec]) & $n=300$ ($t = 3000$ [sec]) & $n=400$ ($t = 4000$ [sec]) & $n=500$ ($t = 5000$ [sec]) \\
    \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5}
    Association (Best-Effort)
        & \raisebox{-.5\height}{\includegraphics[width=.2\linewidth]{Figure_Association/N200.eps}}
        & \raisebox{-.5\height}{\includegraphics[width=.2\linewidth]{Figure_Association/N300.eps}}
        & \raisebox{-.5\height}{\includegraphics[width=.2\linewidth]{Figure_Association/N400.eps}}
        & \raisebox{-.5\height}{\includegraphics[width=.2\linewidth]{Figure_Association/N500.eps}}
        \\
    \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5}
    Trajectory (Best-Effort)
        & \raisebox{-.5\height}{\includegraphics[width=.2\linewidth]{Figure_Trajectory/N200.eps}}
        & \raisebox{-.5\height}{\includegraphics[width=.2\linewidth]{Figure_Trajectory/N300.eps}}
        & \raisebox{-.5\height}{\includegraphics[width=.2\linewidth]{Figure_Trajectory/N400.eps}}
        & \raisebox{-.5\height}{\includegraphics[width=.2\linewidth]{Figure_Trajectory/N500.eps}}
        \\
    \midrule
    & $n=200$ ($t = 2000$ [sec]) & $n=300$ ($t = 3000$ [sec]) & $n=400$ ($t = 4000$ [sec]) & $n=500$ ($t = 5000$ [sec]) \\
    \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5}
    Association (Fairness)
        & \raisebox{-.5\height}{\includegraphics[width=.2\linewidth]{Figure_Association2/N200.eps}}
        & \raisebox{-.5\height}{\includegraphics[width=.2\linewidth]{Figure_Association2/N300.eps}}
        & \raisebox{-.5\height}{\includegraphics[width=.2\linewidth]{Figure_Association2/N400.eps}}
        & \raisebox{-.5\height}{\includegraphics[width=.2\linewidth]{Figure_Association2/N500.eps}}
        \\
    \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5}
    Trajectory (Fairness)
        & \raisebox{-.5\height}{\includegraphics[width=.2\linewidth]{Figure_Trajectory2/N200.eps}}
        & \raisebox{-.5\height}{\includegraphics[width=.2\linewidth]{Figure_Trajectory2/N300.eps}}
        & \raisebox{-.5\height}{\includegraphics[width=.2\linewidth]{Figure_Trajectory2/N400.eps}}
        & \raisebox{-.5\height}{\includegraphics[width=.2\linewidth]{Figure_Trajectory2/N500.eps}}
        \\ 
        % \vspace{-1mm}
    \bottomrule[1pt] 
\end{tabularx}

==> Table/Table_SE.tex <==
\begin{table}\footnotesize
% 	\vspace{.5em}
	\centering
	\caption{Spectral efficiencies under different relaying schemes.} 
	\resizebox{\columnwidth}{!}{\begin{tabular} {l c}
			\toprule[1pt]
			\multirow{2}{*}{\textbf{Relaying Scheme}} & \textbf{Spectral Efficiency} \\
			 & [bits/Hz] \\
			\midrule
			Direct transmission  & \multirow{2}{*}{$ 0.4507 \times 10^{-3}$} \\
			\ without SAT and an additional relays & \\
			SATs & $0.6839 \times 10^{-3}$ \\
			SATs and ground relays & \multirow{2}{*}{$1.9826 \times 10^{-3}$} \\ 
			\ (Association is not optimized) & \\
			SATs and ground relays & \multirow{2}{*}{$18.0727 \times 10^{-3}$} \\
			\ (Association is optimized) & \\
			SATs and UAV relays & \multirow{2}{*}{$\textbf{58.292} \times 10^{-3}$} \\
			\ (\textbf{Proposed EE-Max.}) & \\
			\bottomrule[1pt]
	\end{tabular}}   
% 	\vspace{-1.7em}
	\label{table_SE}
\end{table}
